Code-Aware Prompting: A study of Coverage Guided Test Generation in Regression Setting using LLM

Testing plays a pivotal role in ensuring software quality, yet conventional Search Based Software Testing (SBST) methods often struggle with complex software units, achieving suboptimal test coverage. Recent works using large language models (LLMs) for test generation have focused on improving generation quality through optimizing the test generation context and correcting errors in model outputs, but use fixed prompting strategies that prompt the model to generate tests without additional guidance. As a result LLM-generated testsuites still suffer from low coverage. In this paper, we present SymPrompt, a code-aware prompting strategy for LLMs in test generation. SymPrompt's approach is based on recent work that demonstrates LLMs can solve more complex logical problems when prompted to reason about the problem in a multi-step fashion. We apply this methodology to test generation by deconstructing the testsuite generation process into a multi-stage sequence, each of which is driven by a specific prompt aligned with the execution paths of the method under test, and exposing relevant type and dependency focal context to the model. Our approach enables pretrained LLMs to generate more complete test cases without any additional training. We implement SymPrompt using the TreeSitter parsing framework and evaluate on a benchmark challenging methods from open source Python projects. SymPrompt enhances correct test generations by a factor of 5 and bolsters relative coverage by 26% for CodeGen2. Notably, when applied to GPT-4, SymPrompt improves coverage by over 2x compared to baseline prompting strategies.

==> sections/backups/03_theory.bck.tex <==
\section{Symbolic Path Prompts}

In this section we discuss in details how we collect symbolic paths and leverage them to form the prompts.  




\subsection{Symbolic Path Collection}

\bray{It would be good to give a high level intuition before going into the details}

Algorithm \ref{alg:sympath_generation} describes symbolic path construction. This is performed as follows: \tsc{generateSymbolicPaths} first parses the relevant focal method and then calls \tsc{visitASTNode} on the root of the focal method AST. \tsc{visitASTNode} maintains two lists: \ttt{active\_paths} is a list of possible execution path constraints that must be satisfied to reach the current node in the AST, and \ttt{terminal\_paths}, a list of execution path constraints that terminate at previously visited \ttt{return} statements. Each terminal path is associated with the return value of the return statement where it terminates. ~\bray{We need to emphasize that this process is done statically}

The procedure \tsc{visitASTNode} performs a preorder traversal of the focal method AST.
When \tsc{visitASTNode} visits an AST node, it can do one of three things: if the node is an \ttt{if} or \ttt{while} statement, the visitor will collect relevant constraints and visits the child code blocks of the conditional AST node~\bray{what happens to for loop?}. If the node is a return statement, the visitor will convert all active paths to terminal paths based on the return statement expression. If the the node is neither a conditional statement or return statement, the visitor traverses each of the node children in order.


When the visitor reaches an \ttt{if} statement, it extracts the \ttt{if} condition and visits the \ttt{if} statement's child block with an updated list of active paths that include the if condition. This models the constraints that need to be met in order for any execution to cover the code block under the if statement. After visiting the \ttt{if} child block, the visitor visits each of the \ttt{elif} and \ttt{else} clauses of the \ttt{if} statement while maintaining a negated set of branch constraints from the previously visited clauses in the branch statement. Each \ttt{elif} clause then uses the negated constraints of the previous \ttt{if} and \ttt{elif} that it uses to construct the specific path constraint associated with its child block, while the \ttt{else} clause uses the negated conditions of the \ttt{if} and all \ttt{elif} statements as its path constraint. If the \ttt{if} statement does not have an \ttt{else} clause, a additional path with the negated branch conditions is added to set of active paths to represent the case where the \ttt{if} statement is not executed.   

\gabe{maybe add a detailed walkthrough of how this works on a toy example here. Need to show exactly what path constraints are, how they are collected, otherwise this is pretty confusing}

\ttt{While} statements are treated like \ttt{if} statements, where paths for both the \ttt{while} statement executing at least once, and the \ttt{while} not executing and being skipped, are both added to set of active paths. 
When a \ttt{return} statement is reached, all the active execution paths that reach that return statement are converted into terminal paths with the return statement expression, indicating that these of sets of path constraints that will cause focal method to return the expression in the return statement. 

\todo{add a table or list specifying the definitions of other methods used in the algo that are not formally defined}


\begin{algorithm}
\caption{\label{alg:sympath_generation}Symbolic Path Generation \todo{simplify, formalize}}
\footnotesize
\begin{algorithmic}[1]
\Procedure{generateSymbolicPaths}{focalmethod}
\State root = Parse(focalmethod)
\State active\_paths, terminal\_paths = visitASTNode(root, \{\}, \{\})
\State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, \ttt{None})
\State \Comment{Associates a return value \ttt{None} with each path}
\State \Return terminal\_paths
\EndProcedure
% \State
% \Procedure{addReturnValue}{active\_paths, return\_value}
% \State terminal\_paths = \{\}
% \For{path in active\_paths}
%     \State terminal\_paths $\cap =$ (path, return\_value)
% \EndFor
% \State \Return terminal\_paths
% \EndProcedure
% \State
% \Procedure{addConstraint}{active\_paths, constraint}
% \For{path in active\_paths}
%     \State path = path $\land$ constraint
% \EndFor
% \State \Return active\_paths
% \EndProcedure
\State
\Procedure{visitASTNode}{node, active\_paths, terminal\_paths}
\If{node is an if statement}
    \State if\_constraint = extractConstraint(node)
    \State if\_block = getChildBlock(node)
    \State if\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(if\_block, if\_paths, terminal\_paths)
    \State inv\_constraints = $\neg$if\_constraint)
    \For{child in getChildren(node)}
        \If{child is an elif statement}
            \State elif\_block = getChildBlock(node)
            \State elif\_constraint = extractConstraint(node)
            \State elif\_paths = addConstraint(active\_paths, inv\_constraints $\land \neg$ elif\_constraint)
            \State active\_paths, terminal\_paths = visitASTNode(elif\_block, elif\_paths)
            \State inv\_constraints = inv\_constraints $\cap$ invert(elif\_constraint)
        \ElsIf{child is an else statement}
            \State else\_block = getChildBlock(node)
            \State else\_paths = addConstraint(active\_paths, inv\_constraints)
            \State active\_paths, terminal\_paths = visitASTNode(else\_block, else\_paths)
        \EndIf
    \EndFor
    \If{if node does not have an \ttt{else} child clause}
        \State else\_paths = add\_constraint(active\_paths, inv\_constraints)
        \State active\_paths = active\_paths $\cup$ else\_paths
    \EndIf
\ElsIf{node is a while statement}
    \State while\_constraint = extractConstraint(node)
    \State while\_block = getChildBlock(node)
    \State while\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(while\_block, if\_paths, terminal\_paths)
    \State not\_while\_paths = addConstraint(active\_paths, $\neg$ while\_constraint)
    \State active\_paths = active\_paths $\cup$ not\_while\_paths
\ElsIf{node is a return statement}
    \State return\_value = extractValue(node)
    \State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, return\_value)
    \State active\_paths = \{\}
\Else
    \For{child in getChildren(node)}
        \State active\_paths, terminal\_paths = visitASTNode(child, active\_paths, terminal\_paths)
    \EndFor
\EndIf
\State active\_paths = linearizePaths(active\_paths)
\State \Return active\_paths, terminal\_paths
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Path Linearization}

\begin{algorithm}
\caption{\label{alg:path_linearization}Path Linearization}
\begin{algorithmic}[1]
\footnotesize
\Procedure{linearizePaths}{paths}
\State linearized\_constraints = \{\}
\State linearized\_paths = \{\}
\For{path in paths}
    \State path\_constraints = splitConstraints(path)
    \If{any of path\_constraints is \tbf{not} in linearized\_constraints}
        \State linearized\_constraints = linearized\_constraints $\cap$ path\_constraints
        \State linearized\_paths = linearized\_paths $\cap$ path
    \EndIf
\EndFor
\State \Return linearized\_paths
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{figure}
\centering
        \includegraphics[width=0.6\textwidth]{figures/path_linearize_ex.png}
\caption{Illustration of how path linearization prevents the number of paths from growing exponentially in the number of branches. A method with $n=3$ \ttt{if} conditions will have $2^n = 8$ possible execution paths, but applying Algorithm \ref{alg:path_linearization} reduces the number of paths that need to be tested to at most $n+1 = 4$, each of which covers a unique branch condition.}
\label{fig:path_linearize_ex}
\end{figure}

One challenge in enumerating execution paths in a method is that the number of possible execution paths grows exponentially in the number of branches. Therefore running Algorithm \ref{alg:sympath_generation} on an arbitrary method to collect path constraints can result in a large number of paths to test. This is undesirable because most of the paths will usually not add additional line or branch coverage and therefore are redundant from the perspective of a developer. Therefore, when collecting path constraints to construct symbolic path prompts we only collect a \emph{linearly independent subset} of basis path constraints for use in symbolic prompting.

Basis paths were first proposed as a measure of method complexity~\cite{McCabe1976ACM} and are referred to a basis paths because they form a linear basis for all paths when expressed as a set of columns in the adjacency matrix of the method control-flow-graph. For testing purposes, basis paths are convenient because a set of tests that execute a set of basis paths in a method will achieve full branch coverage on that method.

Algorithm \ref{alg:path_linearization} describes how we compute basis paths from a set of path constraints. We first split each path into its constituent branch constraints, and check if any of the path's constraints are not in the set of linearized path constraints. If a path includes a branch constraint that is not in the linearized constraint set, we add it to the set of linearized paths and add its branch constraints to the set of linearized path constraints. 

Figure \ref{fig:path_linearize_ex} illustrates how path linearization reduces the number of collected paths for a simple example method with three sequential \ttt{if-else} branches. The total number of paths in the method is $2\times2\times2=8$, but applying Algorithm \ref{alg:path_linearization} reduces the number of paths to at most 4 (one initial path, $+1$ for each branch). We apply path linearization in Algorithm \ref{alg:sympath_generation} after \tsc{visitASTNode} is called on any \ttt{if} or \ttt{while} statement that introduces new path constraints.



\subsection{Symbolic Path Prompt Construction}

\begin{figure}
\centering
        \includegraphics[width=0.9\textwidth]{figures/prompt_construction.png}
\caption{Example of symbolic path prompt construction on a simplified focal method in the dataclasses \ttt{Timestamp} class. Each path prompt has three components: \circled{1} \tbf{Method Signature.} The prompt specifies the test case is for the focal method, including its full signature. \circled{2} \tbf{Path Constraints.} Next, the prompt specifies what path constraints should be satisfied by the inputs in the given testcase in order to follow the desired execution path. \circled{3} \tbf{Return Behavior.} The prompt specifies what return behavior, if any, is expected on the specified execution path. This can guide correct generation of assertions for specific return cases.}
\bray{We should give a more complicate example. This looks like we are not doing much.}
\label{fig:prompt_construction}
\end{figure}

Once a set of paths have been collected for a given focal method via Algorithms \ref{alg:sympath_generation} and \ref{alg:path_linearization}, we construct prompts to generate tests for each path based on the focal method signature, path constraints, and return behavior on each collected execution path. Figure \ref{fig:prompt_construction} shows how a prompt is constructed for a single path in a simplified focal method for serializing a timestamp value. Each prompt first specifies the focal method the testcase is for along with the focal method signature, which serves to guide the model to correctly generate the focal method call in the test. The path constraints are joined with \ttt{and}s to indicate that all constraints should be applied when generating the given test case. If the path used to generate the prompt terminates in a return statement, a \ttt{returns: <return\_value>} specifier is added to the prompt to guide assertion generation on the return value.

In many cases method inputs often appear directly in path constraint expressions and return values, as shown in the example in Figure \ref{fig:prompt_construction} where the input \ttt{value} appears in both the path constraint \ttt{isinstance(value, str)} and return expression \ttt{return value}. In these cases the symbolic path prompt provides a direct guide to the construction of the testcase, where input the value should be an instance of \ttt{str} and check the same value is returned. However, we found path prompting is also highly beneficial when path constraints operate on internally defined variables that are set through external method calls such as the \ttt{normalize\_path} call shown in Figure \ref{fig:working_ex_fm}. \gabe{See if we can find a case study with a better example of this for eval and add a forward reference.} 



==> sections/backups/03_theory.tex <==
%\section{Path Constraint Prompts}
\section{Methodology}

% \bray{I'm not sure whether using the term is appropriate here. We are not doing symbolic execution, i.e., not capturing the symbolic values/states. 
% We are kind of traversing each control flow paths and representing them in conditional statements.}

% In this section, we discuss how we construct specialized prompts for test generation that guide the model to generate testcases for a set of execution paths in the focal method that will give full branch and line coverage.

In this section, we elaborate on our approach, \approach, to generate test cases for a given focal method in a regression setting.
At the core of our approach is crafting tailored prompts
that break the problem of test generation into multiple stages of reasoning based on the possible execution paths in focal method. These prompts are designed to instruct the model to generate test cases for a specific set of execution paths within the focal method that will ensure comprehensive branch and line coverage.

% exposing diverse behavior of the underlying focal methods across different execution paths.
%\gabe{@BRAY I modified to framing in terms of full coverage, is that ok?}

\subsection{Overview}

% \bray{I tried to give a generic overview and our reason behing the particular solution. Once we agree on this overview, the rest of the section can be streamlined.}

% We leverage 
Our approach to constructing multi-stage reasoning prompts is based on static symbolic analysis techniques~\cite{godefroid2007compositional, king1976symbolic, baldoni2018survey} to reason about underlying program behavior.  
At a high level, for each control path ($\rho$) of a focal method, 
we statically collect a path constraint $\Phi_\rho$
% ~\bray{are they constrained on input parameters of focal method?}\gabe{no just collected as is w/o any modification} %to describe the input assignments 
that will steer the program execution along $\rho$.

Once the path constraints are collected, in the conventional symbolic analysis-based testing approach, a systematic search algorithm is employed to enumerate all the path constraints~\cite{godefroid2005dart}. 
Feasible paths are those for which the corresponding $\Phi_\rho$ is satisfiable---any concrete solution that meets the conditions of $\Phi_\rho$ can be used to execute and test the path $\rho$ in a regression setting.

However, when dealing with complex real-world code (for instance, when input parameters of the focal method are of complex data types, or when focal methods rely on external dependencies and API calls), the traditional symbolic analysis-based techniques often encounters difficulty in finding a solution. Furthermore, in cases where focal methods feature numerous nested branches and conditions, symbolic execution frequently experiences significant computational overhead.

In this work, we overcome the above mentioned shortcomings in three ways.
First, instead of trying to resolve all the data types and unresolved dependencies while collecting path constraints, we allow approximations. 
For example, if the method \texttt{path.is\_dir()} in Figure~\ref{fig:workflow} cannot be reasoned about symbolically, we leave the condition as it is while collecting $\phi_\rho$. 
Second, to address computational overhead with many branching conditions, we only focus on the paths having unique branching conditions. This design decision significantly helps to reduce the number of paths.
Finally, instead of using a solver to solve the underlying constraints we leverage an LLM to generate test cases based on the collected path constraints. Our insight is that, although the LLM may not reason precisely about all possible constraints, it usually derives enough information from code context and the approximate path constraints %containing variable names and code context 
to generate meaningful test inputs. 


% In traditional symbolic analysis based testing technique~\todo{cite}, 
% a systematic search algorithm enumerates all these path constraints. 
% The feasible paths are those for which the corresponding $\Phi_\rho$ is satisfiable---any solution satisfying $\Phi_\rho$ can be used to execute and test  path $\rho$ in a regression setting. 
% However, in complex real-world code (e.g., input parameters of the focal method are of complex data-types, focal methods have external dependencies and API calls),  traditional symbolic analysis based technique often fails to find a solution. Moreover, focal methods with many nested branches and conditions, symbolic execution often blows up.  

To this end, our prompt generation contains three steps: 
 %At a high level, this involves: 
(Step-I) collecting approximate constraints and return expressions for each path, 
(Step-II) identifying minimal set of paths with unique constraints (i.e., paths that expose new branches), and 
(Step-III) generating prompts amenable to a LLM by leveraging the path constrains identified in the above step.
This entire process is done statically without executing the focal method. 


%\subsection{path constraintCollection}
\subsection{Step-I: Collecting Approximate Path Constraints}

% \todo{objective is to generate test inputs that will follow specific paths. Expose to the model both relevant path constraints and focal method source code and context (type context and dependency context). }

The objective of path constraint prompting is to generate test inputs that will follow specific execution paths in the focal method. To facilitate this, we construct prompts to expose the model both to relevant path constraints, source code of focal method, and type and dependency contexts  that may be necessary to reason about which inputs will satisfy the constraints. In this step, we describe in details how we collected approximate path constraints by statically traversing the abstract parse tree (AST) of the focal method. The detailed algorithm is shown in Algorithm \ref{alg:sympath_generation}.

\begin{algorithm}
\caption{\label{alg:sympath_generation}Path Constraint Collection}
\footnotesize
\begin{algorithmic}[1]
\Procedure{collectPathConstraints}{focalmethod}
\State root = Parse(focalmethod)
\State active\_paths, terminal\_paths = visitASTNode(root, \{\}, \{\})
\State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, \ttt{None})
\State \Comment{Associates a return value \ttt{None} with each path}
\State \Return terminal\_paths
\EndProcedure
% \State
% \Procedure{addReturnValue}{active\_paths, return\_value}
% \State terminal\_paths = \{\}
% \For{path in active\_paths}
%     \State terminal\_paths $\cap =$ (path, return\_value)
% \EndFor
% \State \Return terminal\_paths
% \EndProcedure
% \State
% \Procedure{addConstraint}{active\_paths, constraint}
% \For{path in active\_paths}
%     \State path = path $\land$ constraint
% \EndFor
% \State \Return active\_paths
% \EndProcedure
\State
\Procedure{visitASTNode}{node, active\_paths, terminal\_paths}
\If{node is an if statement}
    \State if\_constraint = extractConstraint(node)
    \State if\_block = getChildBlock(node)
    \State if\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(if\_block, if\_paths, terminal\_paths)
    \State inv\_constraints = $\neg$if\_constraint)
    \For{child in getChildren(node)}
        \If{child is an elif statement}
            \State elif\_block = getChildBlock(node)
            \State elif\_constraint = extractConstraint(node)
            \State elif\_paths = addConstraint(active\_paths, inv\_constraints $\land \neg$ elif\_constraint)
            \State active\_paths, terminal\_paths = visitASTNode(elif\_block, elif\_paths)
            \State inv\_constraints = inv\_constraints $\cap$ invert(elif\_constraint)
        \ElsIf{child is an else statement}
            \State else\_block = getChildBlock(node)
            \State else\_paths = addConstraint(active\_paths, inv\_constraints)
            \State active\_paths, terminal\_paths = visitASTNode(else\_block, else\_paths)
        \EndIf
    \EndFor
    \If{if node does not have an \ttt{else} child clause}
        \State else\_paths = add\_constraint(active\_paths, inv\_constraints)
        \State active\_paths = active\_paths $\cup$ else\_paths
    \EndIf
\ElsIf{node is a while statement}
    \State while\_constraint = extractConstraint(node)
    \State while\_block = getChildBlock(node)
    \State while\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(while\_block, if\_paths, terminal\_paths)
    \State not\_while\_paths = addConstraint(active\_paths, $\neg$ while\_constraint)
    \State active\_paths = active\_paths $\cup$ not\_while\_paths
\ElsIf{node is a return statement}
    \State return\_value = extractValue(node)
    \State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, return\_value)
    \State active\_paths = \{\}
\Else
    \For{child in getChildren(node)}
        \State active\_paths, terminal\_paths = visitASTNode(child, active\_paths, terminal\_paths)
    \EndFor
\EndIf
\State active\_paths = linearizePaths(active\_paths)
\State \Return active\_paths, terminal\_paths
\EndProcedure
\end{algorithmic}
\end{algorithm}

\tsc{collectPathConstraints} first parses the relevant focal method and then calls \tsc{visitASTNode} on the root of the focal method AST. \tsc{visitASTNode} maintains two lists: \ttt{active\_paths} is a list of possible execution path constraints that must be satisfied to reach the current node in the AST, and \ttt{terminal\_paths}, a list of execution path constraints that terminate at previously visited \ttt{return} statements. Each terminal path is associated with the return value of the return statement where it terminates and represented internally as a $(\ttt{path\_constraint}, \ttt{return\_expr})$ tuple.



% This is performed as follows: 
% \tsc{collectPathConstraints} begins by parsing the relevant focal method and subsequently invokes \tsc{visitASTNode} on the root node of the focal method's Abstract Syntax Tree (AST). Within \tsc{visitASTNode}, two lists are maintained: \ttt{active_paths}, which comprises potential execution path constraints necessary to reach the current node in the AST, and \ttt{terminal_paths}, a collection of execution path constraints that conclude at previously encountered \ttt{return} statements. Each terminal path is linked to the return value of the specific \ttt{return} statement where it culminates and is internally represented as a tuple in the form of $(\ttt{path_constraint}, \ttt{return_expr})$.

%\tsc{collectPathConstraints} first parses the relevant focal method and then calls \tsc{visitASTNode} on the root of the focal method AST. \tsc{visitASTNode} maintains two lists: \ttt{active\_paths} is a list of possible execution path constraints that must be satisfied to reach the current node in the AST, and \ttt{terminal\_paths}, a list of execution path constraints that terminate at previously visited \ttt{return} statements. Each terminal path is associated with the return value of the return statement where it terminates and represented internally as a $(\ttt{path\_constraint}, \ttt{return\_expr})$ tuple.

%This is performed as follows: \tsc{collectPathConstraints} first parses the relevant focal method and then calls \tsc{visitASTNode} on the root of the focal method AST. \tsc{visitASTNode} maintains two lists: \ttt{active\_paths} is a list of possible execution path constraints that must be satisfied to reach the current node in the AST, and \ttt{terminal\_paths}, a list of execution path constraints that terminate at previously visited \ttt{return} statements. Each terminal path is associated with the return value of the return statement where it terminates and represented internally as a $(\ttt{path\_constraint}, \ttt{return\_expr})$ tuple.
% ~\bray{We need to emphasize that this process is done statically}\gabe{edited to emphasize}

The procedure \tsc{visitASTNode} performs a preorder traversal of the focal method AST.
When \tsc{visitASTNode} visits an AST node, it can do one of three things: if the node is an \ttt{if} or \ttt{loop} statement, the visitor will collect relevant constraints and visits the child code blocks of the conditional AST node.
% ~\bray{what happens to for loop?} 
If the node is a return statement, the visitor will convert all active paths to terminal paths based on the return statement expression. If the the node is neither a conditional statement or return statement, the visitor traverses each of the node children in order.


When the visitor reaches an \ttt{if} statement, it extracts the \ttt{if} condition and visits the \ttt{if} statement's child block with an updated list of active paths that include the if condition. This models the constraints that need to be met in order for any execution to cover the code block under the if statement. After visiting the \ttt{if} child block, the visitor visits each of the \ttt{elif} and \ttt{else} clauses of the \ttt{if} statement while maintaining a negated set of branch constraints from the previously visited clauses in the branch statement. Each \ttt{elif} clause then uses the negated constraints of the previous \ttt{if} and \ttt{elif} that it uses to construct the specific path constraint associated with its child block, while the \ttt{else} clause uses the negated conditions of the \ttt{if} and all \ttt{elif} statements as its path constraint. If the \ttt{if} statement does not have an \ttt{else} clause, a additional path with the negated branch conditions is added to set of active paths to represent the case where the \ttt{if} statement is not executed.

% \gabe{maybe add a detailed walkthrough of how this works on a toy example here. Need to show exactly what path constraints are, how they are collected, otherwise this is pretty confusing}

\ttt{While} statements are treated like \ttt{if} statements, where paths for both the \ttt{while} statement executing at least once, and the \ttt{while} not executing and being skipped, are both added to set of active paths. 
When a \ttt{return} statement is reached, all the active execution paths that reach that return statement are converted into terminal paths with the return statement expression, indicating that these of sets of path constraints that will cause focal method to return the expression in the return statement. 

% \todo{add a table or list specifying the definitions of other methods used in the algo that are not formally defined}

\begin{comment}
\begin{algorithm}
\caption{\label{alg:sympath_generation}path constraintGeneration \todo{move to appendix/supplemental}}
\footnotesize
\begin{algorithmic}[1]
\Procedure{generateSymbolicPaths}{focalmethod}
\State root = Parse(focalmethod)
\State active\_paths, terminal\_paths = visitASTNode(root, \{\}, \{\})
\State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, \ttt{None})
\State \Comment{Associates a return value \ttt{None} with each path}
\State \Return terminal\_paths
\EndProcedure
% \State
% \Procedure{addReturnValue}{active\_paths, return\_value}
% \State terminal\_paths = \{\}
% \For{path in active\_paths}
%     \State terminal\_paths $\cap =$ (path, return\_value)
% \EndFor
% \State \Return terminal\_paths
% \EndProcedure
% \State
% \Procedure{addConstraint}{active\_paths, constraint}
% \For{path in active\_paths}
%     \State path = path $\land$ constraint
% \EndFor
% \State \Return active\_paths
% \EndProcedure
\State
\Procedure{visitASTNode}{node, active\_paths, terminal\_paths}
\If{node is an if statement}
    \State if\_constraint = extractConstraint(node)
    \State if\_block = getChildBlock(node)
    \State if\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(if\_block, if\_paths, terminal\_paths)
    \State inv\_constraints = $\neg$if\_constraint)
    \For{child in getChildren(node)}
        \If{child is an elif statement}
            \State elif\_block = getChildBlock(node)
            \State elif\_constraint = extractConstraint(node)
            \State elif\_paths = addConstraint(active\_paths, inv\_constraints $\land \neg$ elif\_constraint)
            \State active\_paths, terminal\_paths = visitASTNode(elif\_block, elif\_paths)
            \State inv\_constraints = inv\_constraints $\cap$ invert(elif\_constraint)
        \ElsIf{child is an else statement}
            \State else\_block = getChildBlock(node)
            \State else\_paths = addConstraint(active\_paths, inv\_constraints)
            \State active\_paths, terminal\_paths = visitASTNode(else\_block, else\_paths)
        \EndIf
    \EndFor
    \If{if node does not have an \ttt{else} child clause}
        \State else\_paths = add\_constraint(active\_paths, inv\_constraints)
        \State active\_paths = active\_paths $\cup$ else\_paths
    \EndIf
\ElsIf{node is a while statement}
    \State while\_constraint = extractConstraint(node)
    \State while\_block = getChildBlock(node)
    \State while\_paths = addConstraint(active\_paths, if\_constraint)
    \State active\_paths, terminal\_paths = visitASTNode(while\_block, if\_paths, terminal\_paths)
    \State not\_while\_paths = addConstraint(active\_paths, $\neg$ while\_constraint)
    \State active\_paths = active\_paths $\cup$ not\_while\_paths
\ElsIf{node is a return statement}
    \State return\_value = extractValue(node)
    \State terminal\_paths = terminal\_paths $\cap$ addReturnValue(active\_paths, return\_value)
    \State active\_paths = \{\}
\Else
    \For{child in getChildren(node)}
        \State active\_paths, terminal\_paths = visitASTNode(child, active\_paths, terminal\_paths)
    \EndFor
\EndIf
\State active\_paths = linearizePaths(active\_paths)
\State \Return active\_paths, terminal\_paths
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}

\subsection{Step-II.~Path Minimization}

\begin{algorithm}
\caption{\label{alg:path_minimization}Path Minimization}
\begin{algorithmic}[1]
\footnotesize
\Procedure{minimizePaths}{paths}
\State minimized\_constraints = \{\}
\State minimized\_paths = \{\}
\For{path in paths}
    \State path\_constraints = splitConstraints(path)
    \If{any of path\_constraints is \tbf{not} in minimized\_constraints}
        \State minimized\_constraints = minimized\_constraints $\cap$ path\_constraints
        \State minimized\_paths = minimized\_paths $\cap$ path
    \EndIf
\EndFor
\State \Return minimized\_paths
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{figure}
\centering
        \includegraphics[width=0.6\textwidth]{figures/path_linearize_ex.png}
\caption{Illustration of how path minimization prevents the number of paths from growing exponentially in the number of branches. A method with $n=3$ \ttt{if} conditions will have $2^n = 8$ possible execution paths, but applying Algorithm \ref{alg:path_minimization} reduces the number of paths that need to be tested to at most $n+1 = 4$, each of which covers a unique branch condition.}
\label{fig:path_linearize_ex}
\end{figure}

% \todo{change term to path minimization}

One challenge in enumerating execution paths in a method is that the number of possible execution paths grows exponentially in the number of branches. Therefore running Algorithm \ref{alg:sympath_generation} on an arbitrary method to collect path constraints can result in a large number of paths to test. This is undesirable because most of the paths will usually not add additional line or branch coverage and therefore are redundant from the perspective of a developer. Therefore, when collecting path constraints to construct path constraint prompts we only collect a \emph{linearly independent subset} of basis path constraints for use in prompting.

Basis paths were first proposed as a measure of method complexity~\cite{McCabe1976ACM} and are referred to a basis paths because they form a linear basis for all paths when expressed as a set of columns in the adjacency matrix of the method control-flow-graph. For testing purposes, basis paths are convenient because a set of tests that execute a set of basis paths in a method will achieve full branch coverage on that method.

Algorithm \ref{alg:path_minimization} describes how we compute basis paths from a set of path constraints. We first split each path into its constituent branch constraints, and check if any of the path's constraints are not in the set of linearized path constraints. If a path includes a branch constraint that is not in the linearized constraint set, we add it to the set of linearized paths and add its branch constraints to the set of linearized path constraints. 

Figure \ref{fig:path_linearize_ex} illustrates how path minimization reduces the number of collected paths for a simple example method with three sequential \ttt{if-else} branches. The total number of paths in the method is $2\times2\times2=8$, but applying Algorithm \ref{alg:path_minimization} reduces the number of paths to at most 4 (one initial path, $+1$ for each branch). We apply path minimization in Algorithm \ref{alg:sympath_generation} after \tsc{visitASTNode} is called on any \ttt{if} or \ttt{while} statement that introduces new path constraints.



\subsection{Step-III.~Path Constraint Prompt Construction}

\begin{figure}
\centering
        \includegraphics[width=0.9\textwidth]{figures/prompt_construction.png}
\caption{Example of path constraint prompt construction on a simplified focal method in the \ttt{tornado} project. Each path prompt has three components: \circled{1} \tbf{Method Signature.} The prompt specifies the test case is for the focal method, including its full signature. \circled{2} \tbf{Path Constraints.} Next, the prompt specifies what path constraints should be satisfied by the inputs in the given testcase in order to follow the desired execution path. \circled{3} \tbf{Return Behavior.} The prompt specifies what return behavior, if any, is expected on the specified execution path. This can guide correct generation of assertions for specific return cases.}
% \bray{We should give a more complicate example. This looks like we are not doing much.}\gabe{updated more complex example}
\label{fig:prompt_construction}
\end{figure}

Once a set of path constraints have been collected for a given focal method, 
%via Algorithms \ref{alg:sympath_generation} and \ref{alg:path_linearization}, 
we construct prompts to generate tests for each path based on the focal method signature, path constraints, and return behavior on each collected execution path. Figure \ref{fig:prompt_construction} shows how a prompt is constructed for a single path in a simplified focal method for serializing a timestamp value. Each prompt first specifies the focal method the testcase is for along with the focal method signature, which serves to guide the model to correctly generate the focal method call in the test. The path constraints are joined with \ttt{and}s to indicate that all constraints should be applied when generating the given test case. If the path used to generate the prompt terminates in a return statement, a \ttt{returns: <return\_value>} specifier is added to the prompt to guide assertion generation on the return value.

In many cases method inputs often appear directly in path constraint expressions and return values, as shown in the example in Figure \ref{fig:prompt_construction} where the input \ttt{value} appears in both the path constraint \ttt{isinstance(value, str)} and return expression \ttt{return value}. In these cases the path constraint prompt provides a direct guide to the construction of the testcase, where input the value should be an instance of \ttt{str} and check the same value is returned. However, we found path prompting is also highly beneficial when path constraints operate on internally defined variables that are set through external method calls such as the \ttt{normalize\_path} call shown in Figure \ref{fig:working_ex_fm}. \gabe{See if we can find a case study with a better example of this for eval and add a forward reference.} 



==> sections/backups/04_methodology.tex <==
% not sure if we need this section. 


% \section{Test Generation}


\subsection{Context Construction}

\begin{figure}
\centering
        \includegraphics[width=0.8\textwidth]{figures/adaptive_context.png}
\caption{Illustration of context construction on a focal method \ttt{is\_schema\_valid}. The context is composed of 5 components:
1. \emph{Imports and Globals.} Imported modules and classes that appear in the focal file, along with global variables defined in focal file.
2. \emph{Type Context.} Definitions of types that are used in the focal method and defined in the focal file.
3. \emph{Focal Class Type Context.} The definition of the focal class type signature and initialization.
4. \emph{Focal Class Method Context.} Definitions of any focal class methods that are called in the focal method.
5. \emph{Focal Method.} The definition of the focal method to be tested.
% \begin{enumerate*}
%     \item \emph{Imports and Globals.} Imported modules and classes that appear in the focal file, along with global variables defined in focal file.
%     \item \emph{Type Context.} Definitions of types that are used in the focal method and defined in the focal file.
%     \item \emph{Focal Class Type Context.} The definition of the focal class type signature and initialization.
%     \item \emph{Focal Class Method Context.} Definitions of any focal class methods that are called in the focal method.
% \end{enumerate*}
Constructing the generation context to expose relevant types and dependencies helps the model to attend to relevant definitions when generating. All objects that are included in the context are included in the test execution context and override any import statements generated by the model. This is particularly beneficial for test generations with GPT models, which we found are prone to generating hallucinated import statements (see Section \ref{sec:eval:gpt}).\label{fig:adaptive_context}}
\end{figure}

Prior work in test generation with LLMs have demonstrated that including additional context to the focal method definition is beneficial to the quality of test generations~\cite{tufano2020unit}.
% Athenatest~\cite{tufano2020unit} demonstrated that including focal class signature and focal method/variable signatures improve test generation quality in Java using a small pretrained Transformer, and ChatTester~\cite{yuan2023no} applies similar contexts for test generation with ChatGPT. 
% Codamosa~\cite{lemieux2023codamosa} constructs the generation context \emph{locally} around the focal method by adding lines from the focal file before and after the focal method definition until the context window is fully utilized.
% ChatUniTest~\cite{xie2023chatunitest} constructs an \emph{adaptive} focal context that prioritizes adding class and method definitions to the context that appear in focal method. 
For \approach, we focus on exposing two types of context to the model that are beneficial to generating correct test cases: (i) \emph{Type context.} Context that includes type definitions for focal method parameters guides the model to generate correct test inputs, particularly when the input involves complex data structures. (ii) \emph{Dependency Context.} 
We construct the generation focal context selectively to include only type context and dependency context, but also evaluate as a baseline test generation with a local focal context that is constructed greedily by adding lines from the focal file until the model's input is fully utilized (see Sections \ref{sec:eval:perf_improvement}, \ref{sec:eval:ablation}). 
In addition, we construct the test execution context based on the focal context to override any model-generated imports and type definitions. We found that this prevents many common errors, particularly when generating tests with chat-tuned models such as GPT-4 (See Section \ref{sec:eval:gpt}).

Figure \ref{fig:adaptive_context} illustrates how we construct the generation context. We first parse the focal file and extract all import statements, global definitions, class definitions, and method definitions. We first add all import statements and global definitions to the context. We then check which classes and functions are used in the focal method and add their definitions to the context window if they are defined in the focal file. If the focal method is defined in a class, we extract the class's type signature and constructor definition, and then include the definitions of any methods in the focal class that called in the focal method. Finally, we append the full focal method definition at the end of the context window immediately before the test context and test generation prompt. 



% We found this significantly reduced in errors in generation, particularly with GPT which was prone to generating import statements from hallucinated modules (see Section \ref{sec:eval:gpt}).



\subsection{Test Generation}

\begin{figure}
\centering
        \includegraphics[width=0.9\textwidth]{figures/end2end-cropped.pdf}
\caption{Overview of \approach's framework for test generation. The type and dependency context from the focal method are first parsed from the focal file along with the focal method itself. Path constraint collection is then performed on the focal method. Finally, prompts for each set of path constraints are then constructed passed to the model to generate test cases.\label{fig:end2end}}
\end{figure}

Figure \ref{fig:end2end} gives a high level overview of how we use \approach to generate tests. Given a focal method and it's source file as input, we first collect the relevant dependency and type context. We then collect constraints for a minimal set of execution paths in the focal method that have full branch coverage, and use these to iteratively construct test generation prompts for each path. When generating tests for a set of paths, we iteratively generate tests for each path and include the generated tests in the prompt for the next generation. Following common practice in code generation, for each generation, we check if the output code can be parsed, and if there are parse errors delete lines from the end of the generated code until it parses without errors. This eliminates errors caused by truncated model outputs.


\subsubsection{Prompt Construction}

\begin{figure}
\centering
        \includegraphics[width=0.9\textwidth]{figures/prompt_construction.png}
\caption{Example of path constraint prompt construction on a simplified focal method in the \ttt{tornado} project. Each path prompt has three components: \circled{1} \tbf{Method Signature.} The prompt specifies the test case is for the focal method, including its full signature. \circled{2} \tbf{Path Constraints.} Next, the prompt specifies what path constraints should be satisfied by the inputs in the given testcase in order to follow the desired execution path. \circled{3} \tbf{Return Behavior.} The prompt specifies what return behavior, if any, is expected on the specified execution path. This can guide correct generation of assertions for specific return cases.}
% \bray{We should give a more complicate example. This looks like we are not doing much.}\gabe{updated more complex example}
\label{fig:prompt_construction}
\end{figure}

Once a set of path constraints have been collected for a given focal method, 
%via Algorithms \ref{alg:sympath_generation} and \ref{alg:path_linearization}, 
we construct prompts to generate tests for each path based on the focal method signature, path constraints, and return behavior on each collected execution path. Figure \ref{fig:prompt_construction} shows how a prompt is constructed for a single path in a simplified focal method for serializing a timestamp value. Each prompt first specifies the focal method the testcase is for along with the focal method signature, which serves to guide the model to correctly generate the focal method call in the test. The path constraints are joined with \ttt{and}s to indicate that all constraints should be applied when generating the given test case. If the path used to generate the prompt terminates in a return statement, a \ttt{returns: <return\_value>} specifier is added to the prompt to guide assertion generation on the return value.

% In many cases method inputs often appear directly in path constraint expressions and return values, as shown in the example in Figure \ref{fig:prompt_construction} where the input \ttt{value} appears in both the path constraint \ttt{isinstance(value, str)} and return expression \ttt{return value}. In these cases the path constraint prompt provides a direct guide to the construction of the testcase, where input the value should be an instance of \ttt{str} and check the same value is returned. However, we found path prompting is also highly beneficial when path constraints operate on internally defined variables that are set through external method calls such as the \ttt{normalize\_path} call shown in Figure \ref{fig:working_ex_fm}. 
% \gabe{See if we can find a case study with a better example of this in eval and add a forward reference.} 


\todo{iterative generation here}


We construct the test execution context by importing all defined classes and variables that appear in the generation context. In addition, we copy all of the import statements that appear in the generation context and include them in the execution context. If the model generated any import statements for objects that are imported in the execution context, we remove the model-generated import. 
% \bray{It is not clear what is generation and execution context. Also, in abaltion what is adaptive context?}




